GPT Adoption and the Impact of Disclosure Policies

Generative Pre-trained Transformers (GPTs), particularly Large Language Models (LLMs) like ChatGPT, have proven effective in content generation and productivity enhancement. However, legal risks associated with these tools lead to adoption variance and concealment of AI use within organizations. This study examines the impact of disclosure on ChatGPT adoption in legal, audit and advisory roles in consulting firms through the lens of agency theory. We conducted a survey experiment to evaluate agency costs in the context of unregulated corporate use of ChatGPT, with a particular focus on how mandatory disclosure influences information asymmetry and misaligned interests. Our findings indicate that in the absence of corporate regulations, such as an AI policy, firms may incur agency costs, which can hinder the full benefits of GPT adoption. While disclosure policies reduce information asymmetry, they do not significantly lower overall agency costs due to managers undervaluing analysts' contributions with GPT use. Finally, we examine the scope of existing regulations in Europe and the United States regarding disclosure requirements, explore the sharing of risk and responsibility within firms, and analyze how incentive mechanisms promote responsible AI adoption.

==> JELS/Results/table_authorization.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
& \multicolumn{3}{c}{DV:SecGPTAuth}\\
                                        &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                                        &\multicolumn{1}{c}{No Disclosure}&\multicolumn{1}{c}{Disclosure}&\multicolumn{1}{c}{Whole Sample}\\
\hline
GPTRisk                                 &           -0.420***&            0.084   &           -0.131   \\
                                        &          (0.142)   &          (0.195)   &          (0.111)   \\
[1em]
GPTRisk $\times$ Disclosure             &                    &                    &            0.252** \\
                                        &                    &                    &          (0.114)   \\
[1em]
GPTUsefulness                           &            0.415***&            0.315** &            0.392***\\
                                        &          (0.102)   &          (0.120)   &          (0.061)   \\
[1em]
GPTUsefulness $\times$ Disclosure       &                    &                    &           -0.061   \\
                                        &                    &                    &          (0.061)   \\
[1em]
Disclosure                              &                    &                    &            0.083   \\
                                        &                    &                    &          (0.090)   \\
[1em]
Constant                                &            2.020***&            2.351***&            2.223***\\
                                        &          (0.325)   &          (0.479)   &          (0.282)   \\
\hline
Observations                            &              294   &              258   &              552   \\
Individual controls                     &              Yes   &              Yes   &              Yes   \\
Case fixed-effects                      &              Yes   &              Yes   &              Yes   \\
Pitch section fixed-effects             &              Yes   &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_authorization_align.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                                        &    \multicolumn{3}{c}{DV:SecGPTAuth}        \\
                                        &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                                        &\multicolumn{1}{c}{Whole Sample}&\multicolumn{1}{c}{Less Exp. Managers}&\multicolumn{1}{c}{More Exp. Managers}\\
\hline
\# Avg Prompts $\times$ Disclosure      &            0.019** &            0.024** &            0.012   \\
                                        &          (0.008)   &          (0.010)   &          (0.013)   \\
[1em]
\# Avg Prompts                          &           -0.016   &           -0.013   &           -0.024   \\
                                        &          (0.019)   &          (0.023)   &          (0.033)   \\
[1em]
Constant                                &            2.574***&            2.534***&            2.654***\\
                                        &          (0.064)   &          (0.070)   &          (0.119)   \\
\hline
Observations                            &              552   &              318   &              234   \\
Individual fixed-effects                &              Yes   &              Yes   &              Yes   \\
Case fixed-effects                      &              Yes   &              Yes   &              Yes   \\
Pitch section fixed-effects             &              Yes   &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_authorization_cond.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
& \multicolumn{2}{c}{Dependent variable: SecGPTAuth}\\
\cline{2-3}

                                        &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\hline
GPTUsefulness                           &            0.374***&            0.380***\\
                                        &          (0.063)   &          (0.063)   \\
[1em]
GPTRisk                                 &           -0.251** &           -0.233*  \\
                                        &          (0.124)   &          (0.127)   \\
[1em]
GPTUsefulness $\times$ Disclosure Exp.  &                    &           -0.041   \\
                                        &                    &          (0.064)   \\
[1em]
GPTRisk $\times$ Disclosure Exp.        &                    &            0.136   \\
                                        &                    &          (0.129)   \\
[1em]
Disclosure Exp.                         &                    &            0.063   \\
                                        &                    &          (0.090)   \\
\hline
Observations                            &              552   &              552   \\
Individual controls                     &              Yes   &              Yes   \\
Case fixed-effects                      &              Yes   &              Yes   \\
Pitch section fixed-effects             &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_authorization_experience.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                                        &  \multicolumn{2}{c}{DV: DeckQuality}                     &   \multicolumn{2}{c}{DV:SecGPTAuth}                      \\
                                        &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                                        &\multicolumn{1}{c}{Less Exp. Managers}&\multicolumn{1}{c}{More Exp. Managers}&\multicolumn{1}{c}{Less Exp. Managers}&\multicolumn{1}{c}{More Exp. Managers}\\
\hline
Human-GPT (vs. No-GPT)                  &            0.115*  &            0.153** &                    &                    \\
                                        &          (0.061)   &          (0.073)   &                    &                    \\
[1em]
Human-GPT (vs. No-GPT) $\times$ Disclosure Exp.&           -0.103*  &            0.002   &                    &                    \\
                                        &          (0.061)   &          (0.073)   &                    &                    \\
[1em]
GPTRisk                                 &                    &                    &           -0.195   &           -0.277*  \\
                                        &                    &                    &          (0.166)   &          (0.145)   \\
[1em]
GPTRisk $\times$ Disclosure Exp.        &                    &                    &            0.586***&            0.180   \\
                                        &                    &                    &          (0.186)   &          (0.121)   \\
[1em]
GPTUsefulness                           &                    &                    &            0.351***&            0.467***\\
                                        &                    &                    &          (0.089)   &          (0.081)   \\
[1em]
GPTUsefulness $\times$ Disclosure Exp.  &                    &                    &           -0.166   &           -0.227***\\
                                        &                    &                    &          (0.100)   &          (0.078)   \\
[1em]
Disclosure Exp.                         &                    &                    &            0.016   &           -0.057   \\
                                        &                    &                    &          (0.114)   &          (0.155)   \\
[1em]
Constant                                &            4.292***&            3.918***&            2.596***&            0.968*  \\
                                        &          (0.000)   &          (0.000)   &          (0.484)   &          (0.521)   \\
\hline
Observations                            &              136   &              102   &              318   &              234   \\
Individual fixed-effects                &              Yes   &              Yes   &                    &                    \\
Individual controls                     &                    &                    &              Yes   &              Yes   \\
Case fixed-effects                      &              Yes   &              Yes   &              Yes   &              Yes   \\
Pitch section fixed-effects             &                    &                    &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_authorization_mod.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
& \multicolumn{4}{c}{Dependent variable: SecGPTAuth}\\
\cline{2-5}

                                        &Cont. Quality Hi.   &Cont. Quality Lo.   &  Famil. Case Hi.   &  Famil. Case Lo.   \\
                                        &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   &\multicolumn{1}{c}{(3)}   &\multicolumn{1}{c}{(4)}   \\
\hline
GPTUsefulness                           &            0.314***&            0.355***&            0.403***&            0.251***\\
                                        &          (0.086)   &          (0.116)   &          (0.112)   &          (0.086)   \\
[1em]
GPTRisk                                 &           -0.251   &           -0.360** &           -0.506***&            0.037   \\
                                        &          (0.172)   &          (0.144)   &          (0.157)   &          (0.156)   \\
[1em]
GPTUsefulness $\times$ Disclosure  &           -0.070   &           -0.018   &           -0.024   &           -0.124   \\
                                        &          (0.078)   &          (0.114)   &          (0.083)   &          (0.093)   \\
[1em]
GPTRisk $\times$ Disclosure        &            0.611***&           -0.292*  &           -0.179   &            0.527***\\
                                        &          (0.225)   &          (0.151)   &          (0.142)   &          (0.162)   \\
[1em]
Disclosure                         &            0.127   &            0.006   &           -0.032   &            0.015   \\
                                        &          (0.120)   &          (0.138)   &          (0.151)   &          (0.105)   \\
\hline
Observations                            &              312   &              240   &              216   &              336   \\
Individual controls                     &              Yes   &              Yes   &              Yes   &              Yes   \\
Case fixed-effects                      &              Yes   &              Yes   &              Yes   &              Yes   \\
Pitch section fixed-effects             &              Yes   &              Yes   &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_authorization_qualitygap_mod.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                                        &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                                        &\multicolumn{1}{c}{No Disclosure}&\multicolumn{1}{c}{Disclosure}\\
\hline
GPTRisk                                 &           -0.435***&            0.002   \\
                                        &          (0.129)   &          (0.209)   \\
[1em]
GPTRisk $\times$ IndFavorNoGPTDeck      &           -0.124   &            0.299** \\
                                        &          (0.113)   &          (0.125)   \\
[1em]
GPTUsefulness                           &            0.399***&            0.297***\\
                                        &          (0.105)   &          (0.109)   \\
[1em]
GPTUsefulness $\times$ IndFavorNoGPTDeck&            0.109   &           -0.125   \\
                                        &          (0.106)   &          (0.085)   \\
[1em]
IndFavorNoGPTDeck                       &            0.010   &            0.085   \\
                                        &          (0.104)   &          (0.113)   \\
[1em]
Constant                                &            2.068***&            2.646***\\
                                        &          (0.311)   &          (0.479)   \\
\hline
Observations                            &              294   &              258   \\
Individual controls                     &              Yes   &              Yes   \\
Case fixed-effects                      &              Yes   &              Yes   \\
Pitch section fixed-effects             &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_disclosure.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          DV: DeckQuality   &     DV: $\log$(DeckHour)   &           DV: SecGPTAuth   \\
                         &  \multicolumn{1}{c}{(1)}   &  \multicolumn{1}{c}{(2)}   &  \multicolumn{1}{c}{(3)}   \\
\hline
Human-GPT (vs. No-GPT)   &                    0.169   &                   -0.308***&                            \\
                         &                  (0.132)   &                  (0.075)   &                            \\
[1em]
GPTRisk                  &                            &                            &                    0.078   \\
                         &                            &                            &                  (0.235)   \\
[1em]
GPTUsefulness            &                            &                            &                    0.280***\\
                         &                            &                            &                  (0.073)   \\
[1em]
Constant                 &                    3.944***&                    2.344***&                    2.500***\\
                         &                  (0.066)   &                  (0.038)   &                  (0.509)   \\
\hline
Observations             &                      118   &                      118   &                      258   \\
Individual fixed-effects &                      Yes   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                       No   &                      Yes   \\
Individual controls      &                       No   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_disclosure_cond.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
& \multicolumn{2}{c}{Dependent variable: IndAnalystDisclose}\\
\cline{2-3}
                                        &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\hline
GPTUsefulness                           &            0.308***&            0.268*  \\
                                        &          (0.116)   &          (0.135)   \\
[1em]
GPTRisk                                 &            0.387** &            0.421** \\
                                        &          (0.193)   &          (0.196)   \\
[1em]
GPTUsefulness $\times$ Disclosure Exp.  &                    &            0.082   \\
                                        &                    &          (0.133)   \\
[1em]
GPTRisk $\times$ Disclosure Exp.        &                    &            0.232   \\
                                        &                    &          (0.201)   \\
[1em]
Disclosure Exp.                         &                    &            0.096   \\
                                        &                    &          (0.148)   \\
\hline
Observations                            &               92   &               92   \\
Individual controls                     &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_disclosure_interaction_lessexp.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          DV: DeckQuality   &     DV: $\log$(DeckHour)   &           DV: SecGPTAuth   \\
                         &  \multicolumn{1}{c}{(1)}   &  \multicolumn{1}{c}{(2)}   &  \multicolumn{1}{c}{(3)}   \\
\hline
Human-GPT (vs. No-GPT)   &                    0.343*  &                    0.111   &                            \\
                         &                  (0.180)   &                  (0.088)   &                            \\
[1em]
Human-GPT (vs. No-GPT) $\times$ Disclosure&                   -0.776***&                   -0.323** &                            \\
                         &                  (0.258)   &                  (0.159)   &                            \\
[1em]
IndGPTRisk                  &                            &                            &                   -1.038***\\
                         &                            &                            &                  (0.191)   \\
[1em]
IndGPTUsefulness            &                            &                            &                    0.443***\\
                         &                            &                            &                  (0.122)   \\
[1em]
IndGPTRisk $\times$ Disclosure&                            &                            &                    1.817***\\
                         &                            &                            &                  (0.293)   \\
[1em]
IndGPTUsefulness $\times$ Disclosure&                            &                            &                   -0.458** \\
                         &                            &                            &                  (0.181)   \\
[1em]
Disclosure               &                            &                            &                   -0.057   \\
                         &                            &                            &                  (0.261)   \\
[1em]
Constant                 &                    4.253***&                    2.278***&                    2.651***\\
                         &                  (0.066)   &                  (0.037)   &                  (0.241)   \\
\hline
Observations             &                      108   &                      108   &                      252   \\
Individual fixed-effects &                      Yes   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                       No   &                      Yes   \\
Individual controls      &                       No   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_disclosure_interaction_moreexp.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          DV: DeckQuality   &     DV: $\log$(DeckHour)   &           DV: SecGPTAuth   \\
                         &  \multicolumn{1}{c}{(1)}   &  \multicolumn{1}{c}{(2)}   &  \multicolumn{1}{c}{(3)}   \\
\hline
Human-GPT (vs. No-GPT)   &                    0.449** &                    0.036   &                            \\
                         &                  (0.184)   &                  (0.049)   &                            \\
[1em]
Human-GPT (vs. No-GPT) $\times$ Disclosure&                    0.030   &                   -0.393***&                            \\
                         &                  (0.231)   &                  (0.103)   &                            \\
[1em]
IndGPTRisk                  &                            &                            &                   -0.306   \\
                         &                            &                            &                  (0.184)   \\
[1em]
IndGPTUsefulness            &                            &                            &                    0.537***\\
                         &                            &                            &                  (0.153)   \\
[1em]
IndGPTRisk $\times$ Disclosure&                            &                            &                   -0.188   \\
                         &                            &                            &                  (0.260)   \\
[1em]
IndGPTUsefulness $\times$ Disclosure&                            &                            &                   -0.162   \\
                         &                            &                            &                  (0.184)   \\
[1em]
Disclosure               &                            &                            &                    0.158   \\
                         &                            &                            &                  (0.190)   \\
[1em]
Constant                 &                    3.774***&                    2.293***&                    2.046***\\
                         &                  (0.056)   &                  (0.029)   &                  (0.753)   \\
\hline
Observations             &                      130   &                      130   &                      300   \\
Individual fixed-effects &                      Yes   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                       No   &                      Yes   \\
Individual controls      &                       No   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_disclosure_mod.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
& \multicolumn{4}{c}{Dependent variable: IndAnalystDisclose}\\
\cline{2-5}

                                        &Cont. Quality Hi.   &Cont. Quality Lo.   &  Famil. Case Hi.   &  Famil. Case Lo.   \\
                                        &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   &\multicolumn{1}{c}{(3)}   &\multicolumn{1}{c}{(4)}   \\
\hline
GPTUsefulness                           &            0.580***&           -0.024   &            0.526** &            0.151   \\
                                        &          (0.171)   &          (0.164)   &          (0.255)   &          (0.171)   \\
[1em]
GPTRisk                                 &            0.547** &            0.421*  &            0.241   &            0.717***\\
                                        &          (0.210)   &          (0.226)   &          (0.286)   &          (0.233)   \\
[1em]
GPTUsefulness $\times$ Disclosure  &            0.019   &            0.275   &            0.261   &           -0.069   \\
                                        &          (0.176)   &          (0.173)   &          (0.236)   &          (0.150)   \\
[1em]
GPTRisk $\times$ Disclosure        &            0.553** &            0.069   &           -0.008   &            0.527** \\
                                        &          (0.247)   &          (0.247)   &          (0.278)   &          (0.248)   \\
[1em]
Disclosure                         &            0.046   &            0.083   &            0.050   &            0.053   \\
                                        &          (0.184)   &          (0.249)   &          (0.252)   &          (0.185)   \\
\hline
Observations                            &               44   &               48   &               36   &               56   \\
Individual controls                     &              Yes   &              Yes   &              Yes   &              Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_knowledge_contribution.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                         &\multicolumn{2}{c}{No Disclosure}             
                         &\multicolumn{2}{c}{Disclosure}                            \\
                         \cline{2-3}\cline{4-5} 
                         &\multicolumn{1}{c}{(1)}     &\multicolumn{1}{c}{(2)}     &\multicolumn{1}{c}{(3)}     &\multicolumn{1}{c}{(4)}     \\
                         &\multicolumn{1}{c}{DV: $\log$(DeckHour)}&\multicolumn{1}{c}{DV: SecGPTAuth}&\multicolumn{1}{c}{DV: $\log$(DeckHour)}&\multicolumn{1}{c}{DV: SecGPTAuth}\\
\hline
Human-GPT (vs. No-GPT)   &                    0.091   &                            &                   -0.345***&                            \\
                         &                  (0.056)   &                            &                  (0.081)   &                            \\
[1em]
Human-GPT (vs. No-GPT) $\times$ IndFavorHumanGPTDeck&                    0.120** &                            &                   -0.113   &                            \\
                         &                  (0.056)   &                            &                  (0.081)   &                            \\
[1em]
IndGPTRisk                  &                            &                   -0.389***&                            &                    0.046   \\
                         &                            &                  (0.119)   &                            &                  (0.198)   \\
[1em]
IndGPTUsefulness            &                            &                    0.414***&                            &                    0.313***\\
                         &                            &                  (0.109)   &                            &                  (0.089)   \\
[1em]
IndGPTRisk $\times$ IndFavorHumanGPTDeck&                            &                    0.117   &                            &                   -0.437***\\
                         &                            &                  (0.112)   &                            &                  (0.145)   \\
[1em]
IndGPTUsefulness $\times$ IndFavorHumanGPTDeck&                            &                   -0.108   &                            &                    0.129   \\
                         &                            &                  (0.102)   &                            &                  (0.088)   \\
[1em]
IndFavorHumanGPTDeck     &                            &                    0.049   &                            &                   -0.093   \\
                         &                            &                  (0.099)   &                            &                  (0.116)   \\
[1em]
Constant                 &                    2.230***&                    1.991***&                    2.344***&                    2.974***\\
                         &                  (0.026)   &                  (0.263)   &                  (0.036)   &                  (0.432)   \\
\hline
Observations             &                      120   &                      294   &                      118   &                      258   \\
Individual fixed-effects &                      Yes   &                       No   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                       No   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                      Yes   &                       No   &                      Yes   \\
Individual controls      &                       No   &                      Yes   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_knowledge_contribution_experience.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                         &       Less Exp. Managers   &       More Exp. Managers   \\
                         \cline{2-3}
                         &\multicolumn{1}{c}{(1)}     &\multicolumn{1}{c}{(2)}     \\
                       %  &\multicolumn{1}{c}{DV: SecGPTAuth}&\multicolumn{1}{c}{DV: SecGPTAuth}\\
\hline
IndGPTRisk                  &                   -1.715***&                   -0.071   \\
                         &                  (0.425)   &                  (0.223)   \\
[1em]
IndGPTUsefulness            &                    0.946***&                    0.317***\\
                         &                  (0.211)   &                  (0.100)   \\
[1em]
IndGPTRisk $\times$ IndFavorHumanGPTDeck&                   -1.603***&                   -0.082   \\
                         &                  (0.379)   &                  (0.177)   \\
[1em]
IndGPTUsefulness $\times$ IndFavorHumanGPTDeck&                    0.235   &                    0.041   \\
                         &                  (0.321)   &                  (0.120)   \\
[1em]
IndFavorHumanGPTDeck     &                   -1.155***&                    0.117   \\
                         &                  (0.221)   &                  (0.153)   \\
[1em]
Constant                 &                    0.687   &                    3.612***\\
                         &                  (0.521)   &                  (0.588)   \\
\hline
Observations             &                      126   &                      132   \\
Pitch section fixed-effects&                      Yes   &                      Yes   \\
Individual controls      &                      Yes   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_moderation_gpt_effort.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                         &No Discount in Human Effort   &                            & Discount in Human Effort   &                            \\
                         &\multicolumn{1}{c}{(1)}     &\multicolumn{1}{c}{(2)}     &\multicolumn{1}{c}{(3)}     &\multicolumn{1}{c}{(4)}     \\
                         &\multicolumn{1}{c}{DV: $\log$(DeckHour)}&\multicolumn{1}{c}{DV: SecGPTAuth}&\multicolumn{1}{c}{DV: $\log$(DeckHour)}&\multicolumn{1}{c}{DV: SecGPTAuth}\\
\hline
Human-GPT (vs. No-GPT)   &                   -0.107   &                            &                    0.373*  &                            \\
                         &                  (0.175)   &                            &                  (0.188)   &                            \\
[1em]
Human-GPT (vs. No-GPT) $\times$ Disclosure Exp.&                            &                            &                            &                            \\
                         &                            &                            &                            &                            \\
[1em]
GPTRisk                  &                            &                   -0.219   &                            &                    0.299   \\
                         &                            &                  (0.236)   &                            &                  (0.193)   \\
[1em]
GPTUsefulness            &                            &                    0.451** &                            &                    0.352***\\
                         &                            &                  (0.159)   &                            &                  (0.122)   \\
[1em]
GPTRisk $\times$ Disclosure Exp.&                            &                            &                            &                            \\
                         &                            &                            &                            &                            \\
[1em]
GPTUsefulness $\times$ Disclosure Exp.&                            &                            &                            &                            \\
                         &                            &                            &                            &                            \\
[1em]
Constant                 &                    4.120***&                    1.820** &                    3.814***&                    2.230***\\
                         &                  (0.088)   &                  (0.752)   &                  (0.094)   &                  (0.393)   \\
\hline
Observations             &                       50   &                      114   &                       68   &                      144   \\
Individual fixed-effects &                      Yes   &                       No   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                       No   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                      Yes   &                       No   &                      Yes   \\
Individual controls      &                       No   &                      Yes   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_no_disclosure.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          DV: DeckQuality   &     DV: $\log$(DeckHour)   &           DV: SecGPTAuth   \\
                         &  \multicolumn{1}{c}{(1)}   &  \multicolumn{1}{c}{(2)}   &  \multicolumn{1}{c}{(3)}   \\
\hline
Human-GPT (vs. No-GPT)   &                    0.389***&                    0.079   &                            \\
                         &                  (0.128)   &                  (0.054)   &                            \\
[1em]
GPTRisk                  &                            &                            &                   -0.489***\\
                         &                            &                            &                  (0.162)   \\
[1em]
GPTUsefulness            &                            &                            &                    0.464***\\
                         &                            &                            &                  (0.102)   \\
[1em]
Constant                 &                    4.039***&                    2.230***&                    2.280***\\
                         &                  (0.064)   &                  (0.027)   &                  (0.285)   \\
\hline
Observations             &                      120   &                      120   &                      294   \\
Individual fixed-effects &                      Yes   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                       No   &                      Yes   \\
Individual controls      &                       No   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_no_disclosure_less_experienced.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          DV: DeckQuality   &     DV: $\log$(DeckHour)   &           DV: SecGPTAuth   \\
                         &  \multicolumn{1}{c}{(1)}   &  \multicolumn{1}{c}{(2)}   &  \multicolumn{1}{c}{(3)}   \\
\hline
Human-GPT (vs. No-GPT)   &                    0.400** &                    0.137   &                            \\
                         &                  (0.190)   &                  (0.100)   &                            \\
[1em]
GPTRisk                  &                            &                            &                   -0.692***\\
                         &                            &                            &                  (0.176)   \\
[1em]
GPTUsefulness            &                            &                            &                    0.498***\\
                         &                            &                            &                  (0.154)   \\
[1em]
Constant                 &                    4.089***&                    2.074***&                    4.157***\\
                         &                  (0.095)   &                  (0.050)   &                  (1.275)   \\
\hline
Observations             &                       60   &                       60   &                      138   \\
Individual fixed-effects &                      Yes   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                       No   &                      Yes   \\
Individual controls      &                       No   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_no_disclosure_more_experienced.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          DV: DeckQuality   &     DV: $\log$(DeckHour)   &           DV: SecGPTAuth   \\
                         &  \multicolumn{1}{c}{(1)}   &  \multicolumn{1}{c}{(2)}   &  \multicolumn{1}{c}{(3)}   \\
\hline
Human-GPT (vs. No-GPT)   &                    0.378** &                    0.020   &                            \\
                         &                  (0.183)   &                  (0.045)   &                            \\
[1em]
GPTRisk                  &                            &                            &                   -0.255   \\
                         &                            &                            &                  (0.178)   \\
[1em]
GPTUsefulness            &                            &                            &                    0.499***\\
                         &                            &                            &                  (0.156)   \\
[1em]
Constant                 &                    3.989***&                    2.386***&                    1.633***\\
                         &                  (0.092)   &                  (0.023)   &                  (0.445)   \\
\hline
Observations             &                       60   &                       60   &                      156   \\
Individual fixed-effects &                      Yes   &                      Yes   &                       No   \\
Case fixed-effects       &                      Yes   &                      Yes   &                       No   \\
Pitch section fixed-effects&                       No   &                       No   &                      Yes   \\
Individual controls      &                       No   &                       No   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_quality.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         &          \multicolumn{3}{c}{DV: DeckQuality}          \\
                         \cline{2-4}\\
                         &\multicolumn{1}{c}{(1)}     &\multicolumn{1}{c}{(2)}     &\multicolumn{1}{c}{(3)}     \\
                         &\multicolumn{1}{c}{No Disclosure}&\multicolumn{1}{c}{Disclosure}&\multicolumn{1}{c}{Whole Sample}\\
\hline
Human-GPT (vs. No-GPT)   &                    0.194***&                    0.085   &                    0.140***\\
                         &                  (0.064)   &                  (0.066)   &                  (0.046)   \\
[1em]
Human-GPT (vs. No-GPT) $\times$ Disclosure Exp.&                            &                            &                   -0.055   \\
                         &                            &                            &                  (0.046)   \\
[1em]
Constant                 &                    4.233***&                    4.028***&                    4.132***\\
                         &                  (0.000)   &                  (0.000)   &                  (0.000)   \\
\hline
Observations             &                      120   &                      118   &                      238   \\
Individual fixed-effects &                      Yes   &                      Yes   &                      Yes   \\
Case fixed-effects       &                      Yes   &                      Yes   &                      Yes   \\
\hline\hline
\end{tabular}

}


==> JELS/Results/table_quality_hour.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                         &      \multicolumn{2}{c}{DV: DeckQuality}                                   &       \multicolumn{2}{c}{DV:$\ln$(DeckHour)}                               \\
                         &\multicolumn{1}{c}{(1)}     &\multicolumn{1}{c}{(2)}     &\multicolumn{1}{c}{(3)}     &\multicolumn{1}{c}{(4)}     \\
                         &\multicolumn{1}{c}{No Disclosure}&\multicolumn{1}{c}{Disclosure}&\multicolumn{1}{c}{No Disclosure}&\multicolumn{1}{c}{Disclosure}\\
\hline
Human-GPT (vs. Human)    &                    0.194***&                    0.085   &                    0.039   &                   -0.154***\\
                         &                  (0.064)   &                  (0.066)   &                  (0.027)   &                  (0.038)   \\
[1em]
Constant                 &                    4.233***&                    4.028***&                    2.269***&                    2.190***\\
                         &                  (0.000)   &                  (0.000)   &                  (0.000)   &                  (0.000)   \\
\hline
Observations             &                      120   &                      118   &                      120   &                      118   \\
Individual fixed-effects &                      Yes   &                      Yes   &                      Yes   &                      Yes   \\
Case fixed-effects       &                      Yes   &                      Yes   &                      Yes   &                      Yes   \\
\hline\hline
\end{tabular}
}


==> JELS/Results/table_quality_hour_mod.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                         & \multicolumn{3}{c}{DV: $\log$(DeckHour)}                        \\
                         &\multicolumn{1}{c}{(1)}     &\multicolumn{1}{c}{(2)}     &\multicolumn{1}{c}{(3)}     \\
                         &\multicolumn{1}{c}{No Disclosure}&\multicolumn{1}{c}{Disclosure}&\multicolumn{1}{c}{Whole Sample}\\
\hline
Human-GPT (vs. No-GPT)   &                    0.039   &                   -0.154***&                   -0.057** \\
                         &                  (0.027)   &                  (0.038)   &                  (0.023)   \\
[1em]
Human-GPT (vs. No-GPT) $\times$ Disclosure Exp.&                            &                            &                   -0.097***\\
                         &                            &                            &                  (0.023)   \\
[1em]
Constant                 &                    2.269***&                    2.190***&                    2.230***\\
                         &                  (0.000)   &                  (0.000)   &                  (0.000)   \\
\hline
Observations             &                      120   &                      118   &                      238   \\
Individual fixed-effects &                      Yes   &                      Yes   &                      Yes   \\
Case fixed-effects       &                      Yes   &                      Yes   &                      Yes   \\
\hline\hline
\end{tabular}
}

